One-Step Diffusion Distillation via Deep Equilibrium Models

Diffusion models excel at producing high-quality samples but naively require hundreds of iterations, prompting multiple attempts to distill the generation process into a faster network. However, many existing approaches suffer from a variety of challenges: the process for distillation training can be complex, often requiring multiple training stages, and the resulting models perform poorly when utilized in single-step generative applications. In this paper, we introduce a simple yet effective means of distilling diffusion models directly from initial noise to the resulting image. Of particular importance to our approach is to leverage a new Deep Equilibrium (DEQ) model as the distilled architecture: the Generative Equilibrium Transformer (GET). Our method enables fully offline training with just noise/image pairs from the diffusion model while achieving superior performance compared to existing one-step methods on comparable training budgets. We demonstrate that the DEQ architecture is crucial to this capability, as GET matches a $5\times$ larger ViT in terms of FID scores while striking a critical balance of computational cost and image quality. Code, checkpoints, and datasets are available.

==> sections/table.tex <==
\begin{table*}[th!]
\centering
\begin{minipage}[b]{0.46\textwidth}
    \caption{Generative performance on unconditional CIFAR-10}
    \vspace{-0.15cm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule 
    Method & NFE$\downarrow$ & FID$\downarrow$ & IS$\uparrow$  \\ 
    \midrule
    \gray{Diffusion Models} \\
    \midrule
    DDPM \cite{ddpm}            &  1000 & 3.17 & 9.46  \\
    % DDIM \cite{ddim}            &  1000 & 4.04 & -  \\    
    DDIM \cite{ddim}            &  10 & 13.36 & -  \\
    % Score SDE \cite{score-sde}  & 2000 & 2.2 & 9.89   \\
    % LSGM \cite{lsgm}            &  147 & 2.10 &  \\
    % FastDPM \cite{fastdpm}    &  10 & 9.9 \\
    DPM-solver \cite{dpmsolver} &  10 & 4.7  & -      \\
    DEIS~\cite{deis}            &  10 & 4.17 & -      \\
    EDM~\cite{edm}              &  35 & 2.04 & 9.84   \\ 
    % \midrule
    % \gray{Continuous Flows} \\
    % \midrule
    % 2-ReFlow(+Distill) \cite{reflow} & 1 & 12.21 (4.85) & 8.08 (9.01) \\
    % 3-ReFlow(+Distill) \cite{reflow} & 1 & 8.15 (5.21) & 8.47 (8.79) \\
    % Flow Matching (Diffusion) \cite{flow-matching} &  183 & 8.06 & - \\
    % Flow Matching (OT) \cite{flow-matching}        &  142 & 6.35 & -\\
    % PFGM~\cite{pfgm}                               &  110 & 2.35 &  9.68     \\
    \midrule
    \gray{GANs} \\
    \midrule
    %CR-GAN~\cite{cr-gan}       &  1 & 14.6 & 8.40            \\
    % AutoGAN~\cite{autogan}     &  1 & 12.4 & 8.55            \\
    %ViTGAN~\cite{vitgan}       &  1 & 6.66 & 9.30            \\
    %TransGAN~\cite{transgan}   &  1 & 9.26 & 9.05            \\
    StyleGAN2 \cite{stylegan2} &  1 & 8.32 & 9.18            \\
    %StyleGAN2 + ADA \cite{stylegan2_ada} &  1 & 5.33 & 10.22 \\
    StyleGAN-XL \cite{styleganxl} & 1 & 1.85  & -            \\
    \midrule
    \gray{Diffusion Distillation} \\
    \midrule
     KD~\cite{luhman2021knowledge}      & 1 & 9.36 & 8.36     \\
     PD~\cite{pd}                       & 1 & 9.12 & -        \\
     DSNO~\cite{operator-diffusion}     & 1 & 4.12 & -        \\
     TRACT-EDM~\cite{tract}             & 1 & 4.17 & -        \\
     TRACT~\cite{tract}                 & 1 & 5.02 & -        \\
     PD-EDM~\cite{pd,cm}                & 1 & 8.34 & 8.69     \\
     CD~\cite{cm} & 1 & 3.55 & 9.48  \\
    \midrule
    \gray{Consistency Models}                                \\
    \midrule
    CT~\cite{cm} & 1 & 8.70 & 8.49                           \\
    CT~\cite{cm} & 2 & 5.83 & 8.85                           \\
    \midrule
    \gray{Ours}                                              \\
    \midrule
    GET-Base                  & 1 & 7.42  & 9.16             \\
    GET-Base-2$\times$BS      & 1 & 6.91  & 9.16             \\
    \bottomrule
    \end{tabular}
    }
    % \label{table:unconditional-cifar}
\end{minipage}
\begin{minipage}[b]{0.49\textwidth}
    \caption{Performance of GET architectures on unconditional  CIFAR-10}
    \vspace{-0.08cm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    Models            & Params$\downarrow$ & NFE$\downarrow$ & FID$\downarrow$ & IS$\uparrow$  \\ 
    \midrule
    GET-Mini          & 8.9M  & 1  & 15.19 & 8.37          \\
    GET-Tinier        & 10.3M & 1  & 14.11 & 8.49          \\
    GET-Tiny          & 19.2M & 1  & 10.72 & 8.69          \\
    GET-Small         & 37.2M & 1  & 8.00  & 9.03          \\
    GET-Base          & 62.2M & 1  & 7.42  & 9.16          \\
    GET-Base$+$       & 83.5M & 1  & 7.19  & 9.09          \\
    \midrule
    \gray{Models (More Training)}                                     \\
    \midrule
    GET-Mini-4$\times$Iters            & 8.9M   & 1 & 11.47 & 8.64    \\
    GET-Tinier-4$\times$Iters          & 10.3M  & 1 & 10.79 & 8.76  \\
    GET-Base-2$\times$BS               & 62.2M  & 1 & 6.91  & 9.16    \\
    \bottomrule
    % \label{table:unconditional-cifar-get-arch}
    \end{tabular}
    }
    \vspace{-0.08cm}
    \caption{Generative performance on class-conditional CIFAR-10. $w$ indicates the level of classifier guidance.}
    \vspace{-0.08cm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule 
    Method & NFE $\downarrow$ & FID $\downarrow$ & IS $\uparrow$  \\ 
    \midrule
    \gray{GANs} \\
    \midrule
     BigGAN \cite{biggan} &  1 & 14.73 & 9.22 \\
    % ReACGAN + DiffAug \cite{stylegan_diffaug_d2dce} & 1 & 6.79 & 10.22 \\ 
     StyleGAN2-ADA \cite{stylegan2_ada} & 1 & 2.42 & 10.14 \\
    \midrule
    \gray{Diffusion Models}                \\
    \midrule
     % DDIM \cite{cond-pd} & 2048 & 2.73 & 9.66 \\
     EDM \cite{edm}      & 35   & 1.79 & -    \\
     % NCSN++-G \cite{ncsng} & & 2000 & 2.25 \\
     % EDM-G++ \cite{edmg} & 35 & 1.64 & - \\
    \midrule
    \gray{Diffusion Distillation} \\
    \midrule
    Guided Distillation ($w = 0$) \cite{cond-pd}   &  1 & 8.34  & 8.63    \\
    Guided Distillation ($w = 0.3$) \cite{cond-pd} &  1 &  7.34 & 8.90    \\
    Guided Distillation ($w = 1$) \cite{cond-pd}   &  1 & 8.62  & 9.21    \\
    Guided Distillation ($w = 2$) \cite{cond-pd}   &  1 & 13.23 & 9.23    \\
    \midrule
    \gray{Ours} \\
    \midrule
    GET-Base & 1 & 6.25 & 9.40  \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.15cm}
    % \label{table:conditional-cifar}
\end{minipage}
\end{table*}
